Teacher-Guided Student Self-Knowledge Distillation Using Diffusion Model

Existing Knowledge Distillation (KD) methods often align feature information between teacher and student by exploring meaningful feature processing and loss functions. However, due to the difference in feature distributions between the teacher and student, the student model may learn incompatible information from the teacher. To address this problem, we propose teacher-guided student Diffusion Self-KD, dubbed as DSKD. Instead of the direct teacher-student alignment, we leverage the teacher classifier to guide the sampling process of denoising student features through a light-weight diffusion model. We then propose a novel locality-sensitive hashing (LSH)-guided feature distillation method between the original and denoised student features. The denoised student features encapsulate teacher knowledge and could be regarded as a teacher role. In this way, our DSKD method could eliminate discrepancies in mapping manners and feature distributions between the teacher and student, while learning meaningful knowledge from the teacher. Experiments on visual recognition tasks demonstrate that DSKD significantly outperforms existing KD methods across various models and datasets. Our code is attached in supplementary material.

==> algorithms/training_alg.tex <==
\begin{algorithm*}[t]
    \renewcommand{\baselinestretch}{1.1}
    \caption{\method Basic Alignment (Texture, Shape)}
    \label{alg:data_engine}
    \begin{algorithmic}[1]
    \Require Base model $\pi_0$, quality threshold curriculum $\alpha_k$, ensemble size $N$
    \Ensure Aligned model $\pi_K$ 
    \State {\textbf{//} Let $d = (I, M, S, T, R, t, s)$ denote a demonstration (i.e., a training sample)}
    \For{$k = 1$ to $K$}
        \State {\textbf{// Collection Step:} Generate demonstrations via expert policy}
        \State Initialize $\mathcal{C}_k \leftarrow \emptyset$ \Comment{The dataset collected during iteration $k$}
        \For{$(I, M) \sim p(\mathbf{I},\mathbf{M})$}
            \State $\tilde{\pi}_k \leftarrow \text{Amplify}(\pi_{k-1})$ \Comment{Amplify current policy via model ensemble and best-of-$N$ search}
            \State Sample $\{d_i\}_{i=1}^N \sim \tilde{\pi}_k(I, M)$ \Comment{Generate $N$ candidate demonstrations from expert policy}
            \State $d^*, r \leftarrow \text{HumanRank}(\{d_i\}_{i=1}^N)$ \Comment{Humans select best candidate via pairwise comparisons}
            \State $\mathcal{R} \leftarrow \{d_i : i \neq \arg\max\}$ \Comment{Store rejected candidates for preference learning}
            \State $\mathcal{C}_k \leftarrow \mathcal{C}_k \cup \{(d^*, r, \mathcal{R})\}$ \Comment{Collect chosen demonstration with rating and rejections}
        \EndFor
        \State {\textbf{// Update Step:} Train on aggregated high-quality demonstrations and preferences}
        \State $\mathcal{C} \leftarrow \{(d^+,\mathcal{R}) : (d^+, r, \mathcal{R}) \in \bigcup_{i=1}^k \mathcal{C}_i, r \geq \alpha_k \}$ \Comment{Aggregate and filter by quality}
        \State $\mathcal{D} \leftarrow \{(d^+, d^-) : (d^+, \mathcal{R}) \in \mathcal{C}, d^- \in \mathcal{R}\}$ \Comment{Create preference pairs for DPO training}
        \State $\pi_k^{\text{SFT}} \leftarrow \arg\min_\pi \mathbb{E}_{(d^+, d^-) \sim \mathcal{D}} [\mathcal{L}_{\text{CFM}}(\pi; d^+)]$ \Comment{Supervised finetuning}
        \State $\pi_k \leftarrow \arg\min_\pi \mathbb{E}_{(d^+, d^-) \sim \mathcal{D}} [\mathcal{L}_{\text{DPO}}(\pi, \pi_k^{\text{SFT}}; d^+, d^-)]$ \Comment{Align with preferences}
    \EndFor
    \State \Return $\pi_K$
    \end{algorithmic}
\end{algorithm*}


==> sec/03_training_and_data.tex <==
\section{Training \method}
\label{sec:training}
\method breaks the 3D data barrier using a recipe that progresses from synthetic pretraining to natural post-training, adapting the playbook from LLMs, robotics, and other large generative models. We build capabilities by stacking different training strategies in pre- and mid-training, and then align the model to real data and human-preferred behaviors through a post-training data flywheel.
\method uses the following approach:

\noindent\textbf{Step 1: Pretraining.} This phase builds foundational capabilities, such as shape generation, into a base model.

\noindent\textbf{Step 1.5: Mid-Training.} Sometimes called continued pretraining, mid-training imparts general skills such as occlusion robustness, mask-following, and using visual cues. 

\noindent\textbf{Step 2: Post-Training.} Post-training elicits target behavior, such as adapting the model from synthetic to real-world data or following human aesthetic preferences.
We collect training samples $(I,M)\rightarrow (S,T,R,t,s)$ and preference data from humans and use them in both supervised finetuning (SFT) and direct preference optimization (DPO)~\citep{rafailov2023direct}.

This alignment (step 2) can be repeated, first collecting data with the current model and then improving the model with the new data. This creates a virtuous cycle with humans providing the supervision. \Cref{fig:elo_data_engine} shows that as we run the data engine longer, model performance steadily improves; dataset generation emerges as a byproduct of this alignment.

The following sections detail the training objectives and data sources used in \method. We focus on the Geometry model;  Texture \& Refinement is trained similarly (details  in~\Cref{app:texture_training}). Training hyper-parameters are in~\Cref{sec:training_details}.


\input{figures/sam3d_training_paradigms}

\subsection{Pre \& Mid-Training: Building a Base Model}
\label{section:pretraining_data}

Training begins with synthetic pretraining and mid-training, leveraging available large-scale datasets to learn strong priors for shape and texture, and skills such as mask-following, occlusion handling, and pose estimation. The rich features learned here drastically reduce the number of labeled real-world samples required in post-training~\citep{hernandez2021scaling}, which generally incur acquisition costs.
In pre- and mid-training, models are trained with rectified conditional flow matching~\citep{liu2022flow} to generate multiple 3D modalities (see \Cref{sec:flow_matching_training_objective}).


\subsubsection{Pretraining: Single Isolated 3D Assets}
Pretraining trains the model to reconstruct accurate 3D shapes and textures from renders of isolated synthetic objects, following the successful recipes from~\citep{xiang2025structured,yang2024hunyuan3d,wu2024direct3d}. 
Specifically, we gather a set of image $I$, shape $S$, and texture $T$ triplets, using $2.7$ million object meshes from Objaverse-XL~\citep{deitke2023objaverse} and licensed datasets, and render them from $24$ viewpoints, each producing a high-resolution image of a single centered object; more detail in~\Cref{sec:iso_preprocessing}.
We call this dataset \emph{Iso-3DO} and train for 2.5 trillion training tokens.


\subsubsection{Mid-Training: Semi-Synthetic Capabilities}

Next, mid-training builds up foundational skills that will enable the model to handle objects in real-world images:
\begin{itemize}
    \item \textit{Mask-following}: 
     We train the model to reconstruct a target object, defined by a binary mask on the input image. 
    \item \textit{Occlusion robustness}: 
    The artificial occluders in our dataset incentivize learning shape completion.
    \item \textit{Layout estimation}: We train the model to produce translation and scale in normalized camera coordinates.
\end{itemize}

We construct our data by rendering textured meshes into natural images using alpha compositing.
This ``render-paste'' dataset contains one subset of occluder-occludee pairs, and another subset where we replace real objects with synthetic objects at similar location and scale, creating physically-plausible data with accurate 3D ground truth.  We call this data \emph{RP-3DO}; it contains $61$ million samples with $2.8$ million unique meshes; \Cref{fig:training_data} shows examples.
See~\Cref{app:mid_training_data} for more details.

After mid-training (2.7 trillion training tokens), the model has now been trained with all input and output modalities for visually grounded 3D reconstruction.
However, all data used has been (semi-)synthetic; to both close the domain gap and fully leverage real-world cues, we need real images.

\input{figures/fig_data_engine.tex}


\subsection{Post-Training: Real-World Alignment}
\label{sec:data_engine_alg}
In post-training, we have two goals.  The first is to close the domain gap between (semi-)synthetic data and natural images.  The second is to align with human preference for shape quality.
We adapt the model by using our data engine iteratively; we first \textbf{(i) collect training data} with the current model, and then \textbf{(ii) update our model} using multi-stage post-training on this collected data.  We then repeat.


\subsubsection{Post-Training: Collection Step}
\label{section:data}

The core challenge with collecting data for 3D visual grounding is that most people cannot create meshes directly; this requires skilled 3D artists, who even then can take multiple hours. This is different from the segmentation masks collected in SAM~\citep{kirillov2023segment}.
However, given options, most people \emph{can} choose which mesh resembles an object in the image most accurately. This fact forms the foundation of our data collection for \method.
We convert preferences into training data as follows: sample from our post-trained model, ask annotators to choose the best candidate and then grade its overall quality according to a rubric which we define and update. If the quality meets the (evolving) bar, the candidate becomes a training sample.

Unfortunately at the first iteration, our initial model yields few high-quality candidates. This is because before the first collection step, very little real-world data for 3D visual grounding exists. We deal with this cold start problem by leveraging a suite of existing learned and retrieval-based models to produce candidates.  In early stages, we draw mostly from the ensemble, but as training progresses our best model dominates, eventually producing about $80\%$ of the annotated data seen by \method.

Our annotation pipeline collects 3D object shape $S$, texture $T$, orientation $R$, 3D location $t$, and scale $s$ from real-world images.
We streamline the process by dividing into subtasks and leveraging existing appropriate models and human annotators within each (see \Cref{fig:data_engine}): identifying target objects, 3D model ranking and selection, and posing these within a 3D scene (relative to a point map).
We outline each stage of the data engine below and present details in~\Cref{sec:data_eng_details}. 
In total, we annotate almost $1$ million images with $\sim3.14$ million untextured meshes and $\sim100$K textured meshes--unprecedented scale for 3D data paired with natural images.

\paragraph{Stage 1: Choosing target objects $(I,M)$.}
The goal of this stage is to identify a large, diverse set of images $I$ and object masks $M$ to lift to 3D. 
To ensure generalization across objects and scenes, we sample images from several diverse real-world datasets, and utilize a 3D-oriented taxonomy to balance the object distribution.
To obtain object segmentation masks, we use a combination of pre-existing annotations~\citep{kirillov2023segment} and human labelers selecting objects of interest.

\input{figures/fig_comparison_shape}

\paragraph{Stage 2: Object model ranking and selection $(S,T)$.}
The goal of this stage is to collect image-grounded 3D shape $S$ and texture $T$.  As described above, human annotators choose shape and texture candidates which best match the input image and mask. Annotators rate the example $r$ and reject chosen examples that do not meet a predefined quality threshold, \ie $r < \alpha$. Bad candidates also become negative examples for preference alignment. 

Our data engine maximizes the likelihood of a successful annotation, $r > \alpha$, by asking annotators to choose between $N=8$ candidates from the ensemble; a form of best-of-$N$ search~\citep{ouyang2022training} using humans. The expected quality of this best candidate improves with $N$, and we further increase $N$ by first filtering using a model, and then filtering using the human~\citep{thomas2017exit}; we show results in~\Cref{sec:test_time_search}. 

\paragraph{Stage 2.5: Hard example triage (Artists).}
When no model produces a reasonable object shape, our non-specialist annotators cannot correct the meshes, resulting in a lack of data precisely where the model needs it most.  We route a small percentage of these hardest cases to professional 3D artists for direct annotation, and we denote this set \emph{Art-3DO}. 

\input{figures/fig_comparison_scene}

\paragraph{Stage 3: Aligning objects to 2.5D scene $(R,t,s)$.}
The previous stages produce a 3D shape for the object, but not its layout in the scene.
For each stage 2 shape, annotators label the object pose by manipulating the 3D object's translation, rotation, and scale relative to a point cloud.
We find that point clouds provide enough structure to enable consistent shape placement and orientation. 

In general, we can think of the data collection as an API that takes a current best model, $q(S,T,R,t,s~|~I,M)$, and returns (i) training samples $D^{+} = (I,M,S,T,R,t,s)$, (ii) a quality rating $r\in[0,1]$, and (iii) a set of less preferred candidates ($D^{-} = (I,M,S',T',R',t',s')$) that are all worse than the training sample.

\subsubsection{Post-Training: Model Improvement Step}
The model improvement step in \method uses these training samples and preference results to update the base model through multiple stages of finetuning and preference alignment. 
Within each post-training iteration we aggregate data from all previous collection steps; keeping only samples where $D^{+}$ is above some quality threshold $\alpha$.  As training progresses, $\alpha$ can increase over time, similar to the cross-entropy method for optimization~\citep{2005crossentropymethod}. Our final post-training iteration uses 0.5 trillion training tokens.

\paragraph{Supervised Fine-Tuning (SFT).}
When post-training begins, the base model has only seen synthetic data.  Due to the large domain gap between synthetic and real-world data, we begin by finetuning on our aligned meshes from Stage 3.

We begin SFT with the noisier non-expert labels (MITL-3DO), followed by the smaller, high-quality set from 3D artists (Art-3DO).
The high quality Art-3DO data enhances model quality by aligning outputs with artists' aesthetic preferences. We find this helps suppress common failures, \eg floaters, bottomless meshes, and missing symmetry.

\paragraph{Preference optimization (alignment).}
\label{sec:dpo}
After fine-tuning, the model can robustly generate shape and layout for diverse objects and real-world images.
However, humans are sensitive to properties like symmetry, closure, etc. which are difficult to capture with generic objectives like flow matching.
Thus, we follow SFT with a stage of direct preference optimization (DPO)~\citep{rafailov2023direct}, using $D{+}$/$D^{-}$ pairs from Stage 2 of our data engine.
We found this off-policy data was effective at eliminating undesirable model outputs, even after SFT on Art-3DO. DPO training details are in \Cref{sec:dpo_training_objective}.

\paragraph{Distillation.}
Finally, to enable sub-second shape and layout from the Geometry model, we finish a short distillation stage to reduce the number of function evaluations (NFE) required during inference from $25\rightarrow4$. We adapt~\citet{frans2024one} to our setting, and describe the details in~\Cref{sec:inference}.


==> sec/05_related_work.tex <==
\section{Related Work}
\label{section:related_work}

\paragraph{3D reconstruction} has been a longstanding challenge in computer vision.
Classical methods include binocular stereopsis~\citep{wheatstone1838xviii}, structure-from-motion~\citep{hartley2003multiple,szeliski2022computer,scharstein2002taxonomy,torresani2008nonrigid,tomasi1992shape}, and SLAM~\citep{smith1990estimating,castellanos1999spmap}.
Other strategies reconstruct by analysis (e.g., silhouettes~\citep{esteban2004silhouette}) or by synthesis via volume rendering~\citep{kajiya1984ray}, using either implicit representations~\citep{nerf} or explicit ones~\citep{sitzmann2019deepvoxels,liu2020neural}.
Supervised deep learning methods predict voxels~\citep{xie2019pix2vox,wang2021multi}, point clouds~\citep{van2022revealing}, or meshes~\citep{worchel2022multi,wen2019pixel2mesh++}, 
or optimize implicit representations~\citep{liu2024one}, e.g., signed distance functions (SDFs), often with high-quality output but requiring multiple views at inference.
In contrast, we focus on the more restrictive setting of a single RGB image at test time.

\paragraph{Single-view 3D reconstruction} is considerably more difficult.
A large body of work trains models with direct 3D supervision, predicting meshes~\citep{xu2019disn,kulkarni2021drdf}, voxels~\citep{girdhar2016learning,wu2017marrnet}, point clouds~\citep{fan2017point,mescheder2019occupancy}, or CAD-aligned geometry~\citep{wang2018pixel2mesh,gkioxari2019mesh}.
A recent line of work~\citep{zhang20233dshape2vecset,xiang2025structured,ren2024xcube} supervises with VAE~\citep{kingma2013auto} latent representations.
However, these methods are typically evaluated on simplified synthetic single-object benchmarks such as ShapeNet~\citep{chang2015shapenet}, Pix3D~\citep{sun2018pix3d} or Objaverse~\citep{deitke2023objaverse}.

\paragraph{Layout estimation.}
A large body of work estimates object poses from a single image, for object shapes~\citep{labbe2022megapose,wen2024foundationpose,shi2025sampose,geng2025one,huang2025midi} or detections~\citep{brazil2023omni3d}, but is typically restricted to tabletop robotics, streets, or indoor scenes where objects rest on a supporting surface. In contrast, our approach estimates both pose for a broad range of object types across diverse scenes.

\paragraph{3D datasets.}
Sourcing 3D annotations is challenging: the modality itself is complex, and the specialized tools required are hard to master. Anecdotally, modeling a 3D mesh from a reference image can take an experienced artist hours (\Cref{section:eval}). Instead, existing 3D datasets (\eg, ShapeNet~\citep{chang2015shapenet}, Objaverse-XL~\citep{deitke2023objaverse}) primarily consist of single synthetic objects; without paired real-world images, models can only learn from rendered views. In the real-world domain, existing datasets are small and mostly indoors~\citep{reizenstein2021common,khanna2024habitat,fu20213d,szot2021habitat,pan2023aria}. Models trained on such constrained data struggle to generalize.

\paragraph{Post-training.}
While post-training began with a single supervised finetuning stage~\citep{girshick2014rcnn,wei2021flan}, strong pretraining~\citep{brown2020language} made alignment much more data efficient~\citep{hernandez2021scaling}, enabling iterative preference-based alignment like RLHF~\citep{ouyang2022training} and online DPO~\citep{tang2024understanding, rafailov2023direct}.
When post-training must provide a strong steer, self-training methods offer denser supervision--leveraging the model itself to generate increasingly high-quality demonstrations, rather than relying solely on preference signals~\citep{gulcehre2023reinforcedselftrainingrestlanguage,thomas2017exit,dong2023raft,yuan2023rft}.
\method employs self-training to bridge the synthetic$\rightarrow$real domain gap and break the data barrier for 3D perception; most closely resembling RAFT~\citep{dong2023raft}, but also incorporating preference tuning.

\paragraph{Multi-stage pretraining.}
Modern pretraining increasingly employs multiple training stages. Early work on curriculum learning~\citep{bengio2009curriculum} provided a basis for staged data mixing in pretraining, with higher-quality data coming later~\citep{grattafiori2024llama3herdmodels, olmo20252olmo2furious}. \citet{li2023textbooksneediiphi15,abdin2024phi3technicalreporthighly} show that mixing synthetic/web curricula can achieve strong performance at smaller scales. Increasingly, additional mid-training stages are used for capability injection, such as context extension~\citep{grattafiori2024llama3herdmodels} or coding~\citep{rozière2024codellamaopenfoundation}, and recent work finds that mid-training significantly improves post-training effectiveness~\citep{rlhf2024,wang2025octothinkermidtrainingincentivizesreinforcement}. \method introduces synthetic pretraining and mid-training that can generalize for 3D.


==> sec/acknowledgements.tex <==
\section*{Acknowledgements}
We thank the following individuals for their contributions to this work:

For their contributions to SAM Playground Engineering we thank: Robbie Adkins, Rene de la Fuente, Facundo Figueroa, Alex He, Dex Honsa, Alex Lende, Jonny Li, Peter Park, Don Pinkus, Roman Radle, Phillip Thomas, and Meng Wang.  We thank our excellent XFN team for leadership and support: Kris Kitani, Vivian Lee, Sasha Mitts, George Orlin, Nikhila Ravi, and Andrew Westbury.  Thanks to Helen Klein, Mallika Malhotra, and Azita Shokrpour for support with Legal, Privacy, and Integrity.  We thank Michelle Chan, Kei Koyama, William Ngan, Yael Yungster for all the design support throughout the project.  Thanks to Arpit Kalla for work on model efficiency.  We thank Faye Ma and Kehan Lyu for data engineering support and tooling, and Emmanuel Hernandez, Robert Kuo for pipeline development.  We thank Nan Yang for support with egocentric video data efforts.  Thanks to our two interns Cem Gokmen, Jasmine Shone for their work on 3D and Lea Wilken for feedback on the manuscript. Thanks to our fantastic data operations team: Paris Baptiste, Karen Bergan, Kai Brown, Ida Cheng, Khadijat Durojaiye, Patrick Edwards, Daniella Factor, Eva Galper, Leonna Jones, Zayida Suber, Tatum Turner, Joseph Walker, and Claudette Ward.


==> tables/table_ablation_stage.tex <==

\begin{table}[ht!]
    \centering
        \begin{NiceTabular}{llcccc}
        \CodeBefore
        \Body
        \toprule
        &   & \multicolumn{4}{c}{SA-3DAO} \\
        \cmidrule(lr){3-6}
        Model  &  Training Setup   & F1 @ 0.01 ($\uparrow$) & vIoU ($\uparrow$)  & Chamfer ($\downarrow$) & EMD ($\downarrow$) \\
        \midrule
        \method & Full & \textbf{0.2344} & \textbf{0.2311} & \textbf{0.0400} & \textbf{0.1211} \\
                & w/o training on MITL-3DO & 0.2211 & 0.2220 & 0.0486 & 0.1338 \\
                & w/o training on Art-3DO & 0.2027 & 0.2025 & 0.0578 & 0.1510 \\
                & w/o DPO on MITL-3DO & 0.2156 & 0.2156 & 0.0498 & 0.1367 \\
        \bottomrule
        \end{NiceTabular}
    \caption{\textbf{Training stage knockout.} The impact of training on MITL and 3D artist-generated data.}
    \label{table:ablate_stage}
\end{table}

==> tables/table_all_stage.tex <==
\begin{table}[t]
    \centering
        \begin{NiceTabular}{lccccc}
        \CodeBefore
        \Body
        \toprule
        & \multicolumn{4}{c}{SA-3DAO} & Preference set \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-6}
        Training Stage   & F1 @ 0.01 ($\uparrow$) & vIoU ($\uparrow$) & Chamfer ($\downarrow$) & EMD ($\downarrow$)  & Texture WR ($\uparrow$) \\
        \midrule
        Pre-training (Iso-3DO) & 0.1349 & 0.1202 & 0.1036 & 0.2396 & - \\
        + Mid-training (RP-3DO) &  0.1705 & 0.1683 & 0.0760 & 0.1821 & 60.7 \\
        + SFT (MITL-3DO) & 0.2027 & 0.2025 & 0.0578 & 0.1510 & 66.9 \\
        + DPO (MITL-3DO) & 0.2156 & 0.2156 & 0.0498 & 0.1367 & 66.4 \\
        + SFT (Art-3DO)  & 0.2331 & \textbf{0.2337} & 0.0445 & 0.1257 & - \\
        + DPO (Art-3DO) & \textbf{0.2344} & 0.2311 & \textbf{0.0400} & \textbf{0.1211} & - \\
        \bottomrule
        \end{NiceTabular}
    \caption{\textbf{Cascading improvements from multi-stage training on 3D shape and texture}. 
    For texture, we report win rates (WR) between each row and the row \textit{above} it.}
    \label{table:stage}
\end{table}


==> tables/table_comparison_layout.tex <==
\begin{table*}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
        \begin{NiceTabular}{clcccccccc}
        \CodeBefore
        \Body
        \toprule
            & &  \multicolumn{4}{c}{SA-3DAO} & \multicolumn{4}{c}{Aria Digital Twin} \\
        \cmidrule(lr){3-6} \cmidrule(lr){7-10}
        Generation & Model   & 3D IoU ($\uparrow$) & ICP-Rot. ($\downarrow$) & ADD-S ($\downarrow$) & ADD-S @ 0.1 ($\uparrow$) & 3D IoU ($\uparrow$) & ICP-Rot. ($\downarrow$) & ADD-S ($\downarrow$) & ADD-S @ 0.1 ($\uparrow$)   \\
        \midrule
         Pipeline & Trellis + Megapose & 0.2449 & 39.3866 & 0.5391 & 0.2831 & 0.2531 & 33.6114 & 0.4358 & 0.1971  \\         
         Pipeline & HY3D-2.0 + Megapose & 0.2518 & 33.8307 & 0.7146 & 0.3647 & 0.3794 & 29.0066 & 0.1457 & 0.4211  \\         
         Pipeline & HY3D-2.0 + FoundationPose & 0.2937 & 32.9444 & 0.3705 & 0.5396 & 0.3864 & 25.1435 & 0.1026 & 0.5992  \\
         Pipeline & HY3D-2.1 + FoundationPose & 0.2395 & 39.8357 & 0.4186 & 0.4177 & 0.2795 & 33.1197 & 0.2135 & 0.4129  \\
         Pipeline & \method + FoundationPose  & 0.2837 & 32.9168 & 0.3848 & 0.5079 & 0.3661 & 18.9102 & 0.0930 & 0.6495  \\
         \addlinespace[0.5em]
         Joint & MIDI & - & - & - & - & 0.0336 & 44.2353 & 2.5278 & 0.0175  \\         
         \midrule
         Joint & \textbf{\method} & \textbf{0.4254} & \textbf{20.7667} & \textbf{0.2661} & \textbf{0.7232} & \textbf{0.4970} & \textbf{15.2515} & \textbf{0.0765} & \textbf{0.7673} \\
        \bottomrule
        \end{NiceTabular}
    } 
    \caption{\textbf{3D layout quantitative comparison} to competing layout prediction methods on SA-3DAO and Aria Digital Twin~\citep{pan2023aria}. \method significantly outperforms both \emph{pipeline} approaches used in robotics~\citep{labbe2022megapose,wen2024foundationpose} and \emph{joint} generative models (MIDI~\citep{huang2025midi}). Most SA-3DAO scenes only contain one object so we do not show MIDI results that require multi-object alignment. The metrics measure bounding box overlap, rotation error, and chamfer-like distances normalized by object diameter.
    }
    \label{table:comparison_layout}
\end{table*}

==> tables/table_comparison_metrics.tex <==
\begin{table}[t]
    \centering
        \begin{NiceTabular}{lcccccc}
        \CodeBefore
        \Body
        \toprule
            & \multicolumn{4}{c}{SA-3DAO} & \multicolumn{2}{c}{ISO3D Eval Set} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}
        Model 
            & F1@0.01 ($\uparrow$) 
            & vIoU ($\uparrow$) 
            & Chamfer ($\downarrow$)  
            & EMD ($\downarrow$)
            & ULIP ($\uparrow$) 
            & Uni3D ($\uparrow$)  \\
            
        \midrule
         Trellis
            & 0.1475 & 0.1392 & 0.0902 & 0.2131
            & 0.1473 & 0.3698\\
         HY3D-2.1
            & 0.1399 & 0.1266 & 0.1126 & 0.2432
            & 0.1293 & 0.3546 \\
         HY3D-2.0
            & 0.1574 & 0.1504 & 0.0866 & 0.2049
            & 0.1484 & 0.3662 \\
         Direct3D-S2 
            & 0.1513 & 0.1465 & 0.0962 & 0.2160
            & 0.1405 & 0.3653 \\
         TripoSG
            & 0.1533 & 0.1445 & 0.0844 & 0.2057 
            & \textbf{0.1529} & 0.3687 \\
         Hi3DGen
            & 0.1629 & 0.1531 & 0.0937 & 0.2134 
            & 0.1419 & 0.3594 \\
        \midrule 
        \textbf{\method} 
            & \textbf{0.2344} & \textbf{0.2311} & \textbf{0.0400} & \textbf{0.1211}
            & 0.1488 & \textbf{0.3707}\\
        \bottomrule
        \end{NiceTabular}
    \caption{\textbf{3D shape quantitative comparison} to competing image-to-3D methods, including Trellis~\citep{xiang2025structured}, HY3D-2.1~\citep{hunyuan3d2025hunyuan3d}, HY3D-2.0~\citep{hunyuan3d22025tencent}, Direct3D-S2~\citep{wu2025direct3ds2gigascale3dgeneration}, TripoSG~\citep{li2025triposg}, Hi3DGen~\citep{ye2025hi3dgen}.
    SA-3DAO shows metrics that measure accuracy against GT geometry; ISO3D~\citep{ebert20253d} has no geometric GT and so we show perceptual similarities between 3D and input images (ULIP~\citep{xue2023ulip} and Uni3D~\citep{zhou2023uni3d}). TripoSG uses a significantly higher mesh resolution, which is rewarded in perceptual metrics.
    }
    \label{table:comparison_shape}
\end{table}


==> tables/table_comparison_post-optim_layout.tex <==
  \begin{table*}[h]
      \centering
      \resizebox{0.7\textwidth}{!}{
          \begin{NiceTabular}{lccccc}
          \CodeBefore
          \Body
          \toprule
          Model   & 3D IoU ($\uparrow$) & ICP-Rot. ($\downarrow$) & ADD-S ($\downarrow$) & ADD-S @ 0.1 ($\uparrow$) & 2D IoU ($\uparrow$) \\
          \midrule
          \method & 0.4837 & 14.4702 & 0.08265 & 0.7545 & 0.5143 \\
          \method~(post-optim) & \textbf{0.5258} & \textbf{14.1460} & \textbf{0.07932} & \textbf{0.7617} & \textbf{0.6487} \\
          \bottomrule
          \end{NiceTabular}
      } 
      \caption{\textbf{Test-time optimization for layout.} Quantitative comparison of \method layout test-time optimization on Aria Digital Twin~\citep{pan2023aria}.}
      \label{table:comparison_post-optim}
  \end{table*}


==> tables/table_comparison_texture.tex <==
\begin{figure}[ht!]
    \centering
    \begin{minipage}[c]{0.48\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \begin{NiceTabular}{lcccc}
            \CodeBefore
            \Body
            \toprule
            & \multicolumn{4}{c}{\method WR over baselines, \method shape} \\
            \cmidrule(lr){2-5}
            Model & iso3d & Preference Set & SA-3DAO & LVIS \\
            \midrule 
            Trellis & 81.1 & 87.0 & 86.2 & 89.1 \\
            Hunyuan3D-2.1 & 63.8 & 87.0 & 86.2 & 89.1 \\
            Hunyuan3D-2.0 & 70.1  & 77.5 & 77.4 & 85.7 \\
            Unitex & 83.3 & 84.7 & 84.5 & 88.3 \\
            \bottomrule
            \end{NiceTabular}
        }
        \captionof{table}{\textbf{3D texture.} Preference results comparing \method to competing image-to-3D methods on ISO3D~\citep{ebert20253d}, Preference Set, and SA-3DAO. We compare to the recent Trellis~\citep{xiang2025structured}, Hunyuan3D-2.1~\citep{hunyuan3d2025hunyuan3d}, and Unitex~\citep{liang2025unitex}, with the same shape of \method. The human preference rates represent preference for \method over each baseline approach.}
        \label{table:comparison_texture}
    \end{minipage}
    \hfill 
    \begin{minipage}[c]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig_texture_ablations.png}
        \caption{\textbf{Ablations for the Texture \& Refinement model, grouped by training stage.} Percentages denote human preference rate for each ablation, over the model \textit{without} the ablation.}
        \label{fig:ablations_texture}
    \end{minipage}
\end{figure}

==> tables/table_distillation.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}[b]{0.94\textwidth}
\centering 
\includegraphics[width=\textwidth]{figures/stage1_distillation.png}
\label{fig:preference:subfig1}
\end{subfigure}
\vspace{-0.5cm}
\caption{\textbf{Model distillation.} Geometry model shortcut versus flow matching. Flow matching distillation enables the model to perform significantly better during the early iterations, nearly on par with 25 steps performance.} 
\label{fig:distillation}
\end{figure}

==> tables/table_training_hyperparameters_geometry.tex <==
\begin{table*}[t!]
\centering
\label{table:training_hyperparameters}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
\textbf{Training stage} & \textbf{Datasets} & \textbf{Condition input} & \textbf{Learning rate} & \textbf{Modality weights} & \textbf{\# Meshes} & \textbf{\# Images} & \textbf{\# Samples} & \textbf{\# Tokens} \\
\midrule
Pre-training & Iso-3DO & object-centric crop & $10^{-4}$ & $S{=}1.0, R{=}0.1$ & 2.7M & 64.8M & 64.8M & 2.5T \\
\multirow{2}{*}[0mm]{Mid-training}
    & RP-3DO (FO)& full image & $10^{-4}$ & $S{=}1.0, R{=}0.1$ & 2.87M & 11.17M & 55.1M & 2.4T \\
    & RP-3DO (OS-R), ProcThor & full image, pointmap & $10^{-4}$ & $S{=}1.0, R{=}0.1, t{=}1.0, s{=}0.1$ & 2.38M & 1.20M & 5.95M & 0.3T \\
SFT & MITL-3DO, Art-3DO & full image, pointmap & $10^{-5}$ & $S{=}1.0, R{=}0.1, t{=}1.0, s{=}0.1$ & 0.6M & 0.5M & 0.6M & 0.9T \\
Alignment & MITL preference & full image, pointmap & $2.5\times10^{-6}$ & $S{=}1.0$ & 88K & 31K & 44K & - \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Detailed training hyperparameters for SAM 3D training stages (Geometry Model)}. This table extends Table 1 from the main paper with additional hyperparameter details.}
\label{table:geometry_model_training_details}
\end{table*}

==> tables/table_training_hyperparameters_texture.tex <==
\begin{table*}[t!]
\centering
\label{table:texture_training_hyperparameters}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
\textbf{Training stage} & \textbf{Datasets} & \textbf{Condition input} & \textbf{Learning rate} & \textbf{EMA} & \textbf{\# Meshes} & \textbf{\# Images} & \textbf{\# Samples} & \textbf{\# Tokens} \\
\midrule
Pre-training & Trellis500K & object-centric crop & $10^{-4}$ & 0.9999 & 350K & 9M & 10M & 1.1T \\
Mid-training & RP-3DO (FO,OS-A) & full image & $10^{-4}$ & 0.9999 & 800K & 2.4M & 2.4M & 1T \\
SFT & MITL & full image & $10^{-5}$ & 0.999 & $\sim$100K & 100K & 100K & 115B \\
Alignment & MITL preference & full image & $10^{-6}$ & 0.99 & 146K & 73K & 73K & - \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Detailed training hyperparameters for SAM 3D training stages (Texture \& Refinement Model).} This table extends Table 1 from the main paper with additional hyperparameter details.}
\label{table:texture_model_training_details}
\end{table*}

==> tables/table_vlm_search.tex <==
\begin{table}[h]
\centering
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
& \multicolumn{2}{c|}{Tail Holdout} & \multicolumn{2}{c|}{Epic Kitchens} & \multicolumn{2}{c}{SA-3DAO} \\
& Chamfer $\downarrow$ & F1 $\uparrow$ & Chamfer $\downarrow$ & F1 $\uparrow$ & Chamfer $\downarrow$ & F1 $\uparrow$ \\
\midrule
SFT with $N=2$ & 0.0059 & 0.39 & 0.0094 & 0.30 & 0.0083 & 0.26 \\
SFT with $N=50$ recovery & \textbf{0.0053} & \textbf{0.41} & \textbf{0.0090} & \textbf{0.32} & \textbf{0.0081} & \textbf{0.26} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Including reward-model-recovered data during SFT}, from the pipeline in \Cref{fig:vlm_search}, improves model performance on challenging inputs, as seen in both Chamfer Distance and F1 score on the tail holdout set, Epic Kitchens~\citep{damen2020epic}, and SA-3DAO.}
\label{table:vlm_search}
\end{table}
